Parcel loss prediction in last-mile delivery: deep and non-deep approaches with insights from Explainable AI

Within the domain of e-commerce retail, an important objective is the reduction of parcel loss during the last-mile delivery phase. The ever-increasing availability of data, including product, customer, and order information, has made it possible for the application of machine learning in parcel loss prediction. However, a significant challenge arises from the inherent imbalance in the data, i.e., only a very low percentage of parcels are lost. In this paper, we propose two machine learning approaches, namely, Data Balance with Supervised Learning (DBSL) and Deep Hybrid Ensemble Learning (DHEL), to accurately predict parcel loss. The practical implication of such predictions is their value in aiding e-commerce retailers in optimizing insurance-related decision-making policies. We conduct a comprehensive evaluation of the proposed machine learning models using one year data from Belgian shipments. The findings show that the DHEL model, which combines a feed-forward autoencoder with a random forest, achieves the highest classification performance. Furthermore, we use the techniques from Explainable AI (XAI) to illustrate how prediction models can be used in enhancing business processes and augmenting the overall value proposition for e-commerce retailers in the last mile delivery.

==> Preface.tex <==
This master thesis is the final piece of work of my Master in Science in Operations Management \& Logistics. This report marks the end of my life as a student. A period I have truly enjoyed and on which I can look back with a big smile on my face. I want to express my gratitude to everyone who has been involved in my student life. I am really thankful for my family and friends, especially throughout the world-wide COVID-19 pandemic.\\

Furthermore, I would like to thank my mentor and first supervisor, Yingqian Zhang. Thanks for your involvement, all the structural feedback and the confidence in my capabilities to deep-dive into this master thesis project. I would also like to thank Laurens Bliek for your contributions to this master thesis. \\

Finally, I would like to thank Coolblue and everyone from the Delivery Partners department. I have learned a lot and enjoyed working with you at the office in Rotterdam. However, I would like to thank some persons in particular. To my company supervisor, Lyanne Bakker, I would like to thank you for giving me this wonderful opportunity and guiding me throughout the project. Furthermore, my fellow analysts, Gijs Koendes, Rohit Shah and Taru van der Zijde. I would like to thank you for your time, continuous support, our fantastic activities and making me start every day with a smile. I have learned a lot from you and will never forget this wonderful period. \\

\begin{flushright}
    Jan de Leeuw \\
    Eindhoven, October 2022
\end{flushright}


